Towards Adaptive Training of Agent-based Sparring Partners for Fighter Pilots

A key requirement for the current generation of artificial decision-makers is that they should adapt well to changes in unexpected situations. This paper addresses the situation in which an AI for aerial dog fighting, with tunable parameters that govern its behavior, must optimize behavior with respect to an objective function that is evaluated and learned through simulations. Bayesian optimization with a Gaussian Process surrogate is used as the method for investigating the objective function. One key benefit is that during optimization, the Gaussian Process learns a global estimate of the true objective function, with predicted outcomes and a statistical measure of confidence in areas that haven't been investigated yet. Having a model of the objective function is important for being able to understand possible outcomes in the decision space; for example this is crucial for training and providing feedback to human pilots. However, standard Bayesian optimization does not perform consistently or provide an accurate Gaussian Process surrogate function for highly volatile objective functions. We treat these problems by introducing a novel sampling technique called Hybrid Repeat/Multi-point Sampling. This technique gives the AI ability to learn optimum behaviors in a highly uncertain environment. More importantly, it not only improves the reliability of the optimization, but also creates a better model of the entire objective surface. With this improved model the agent is equipped to more accurately/efficiently predict performance in unexplored scenarios.

==> Conclusion.tex <==
\section{Conclusion}
Talk about the main themes of the paper. Possibly combine this section with the discussion.


==> Experimental_setup.tex <==
\subsection{ExperimentalSetup}
Two agents were placed in a simulated engagement. The behavioral parameters of one agent was held constant, the parameters of the other agent were chosen by using Bayesian optimization. The simulation environment used was called ``MSS'' which is a product made by Orbit Logic Inc. During each engagement key metrics were tracked and then provided to the Bayesian optimization algorithm.

